Impacts and Risk of Generative AI Technology on Cyber Defense

Generative Artificial Intelligence (GenAI) has emerged as a powerful technology capable of autonomously producing highly realistic content in various domains, such as text, images, audio, and videos. With its potential for positive applications in creative arts, content generation, virtual assistants, and data synthesis, GenAI has garnered significant attention and adoption. However, the increasing adoption of GenAI raises concerns about its potential misuse for crafting convincing phishing emails, generating disinformation through deepfake videos, and spreading misinformation via authentic-looking social media posts, posing a new set of challenges and risks in the realm of cybersecurity. To combat the threats posed by GenAI, we propose leveraging the Cyber Kill Chain (CKC) to understand the lifecycle of cyberattacks, as a foundational model for cyber defense. This paper aims to provide a comprehensive analysis of the risk areas introduced by the offensive use of GenAI techniques in each phase of the CKC framework. We also analyze the strategies employed by threat actors and examine their utilization throughout different phases of the CKC, highlighting the implications for cyber defense. Additionally, we propose GenAI-enabled defense strategies that are both attack-aware and adaptive. These strategies encompass various techniques such as detection, deception, and adversarial training, among others, aiming to effectively mitigate the risks posed by GenAI-induced cyber threats.

==> commented.tex <==
\begin{comment}
\IEEEPARstart{A}{}ttacks against digital information, whether in the form of information at rest or information in motion, continue to grow in number, severity, and importance.
The Internet evolved from a scholarly curiosity to a central place in almost everyone's everyday existence who utilizes or is impacted by modern technology.
Hackers quickly recognized the importance of the information on the Internet as well as how much society relied on the connectivity and communications that networks afforded.
Cyber-attacks pose an ongoing threat to users' digital lives and are increasingly sophisticated, owing to advanced technological countries focusing heavier on acquiring and fortifying their cyber-offensive and defensive capabilities. 
In \cite{}, Dutta et al. indicated that devices and networks are vulnerable to severe attacks that can negatively impact user's daily lives.
Complex intrusions are being developed with sophisticated algorithms that are able to bypass detection systems that are not sophisticated enough to deal with the complexity of threats in today's networks.
Information about the user’s digital life can be stored, analyzed to plan further attacks, and/or sold by the attackers. 
Often these compromised systems are combined with other compromised systems to attack more targets in what becomes a snowballing action. 
These threats and the lack of robust detection systems leave sensitive data exposed.
Protecting systems and networks from these attacks is a major cybersecurity goal. 
Although security systems are improving their resistance and security as a result of training for a wider variety of attacks, there remain various attacks that are not covered. 
Moreover, attacks are discovered with regularity. 
Thus, the question may be asked, if the defender does not know that an attack exists, how can they protect against such an attack? 
As a result, detection systems are used to protect networks against only known attacks. 
What follows are several examples [4] of attacks on systems that have failed to provide adequate protection, which motivated this survey:



\subash{Trim this paragraph.... If you can restructure introduction to following strcucture that would be great}
\hl{Introduction Flow:}
\begin{itemize}
    
\item 
Second Para
-	Describe how attacks impact critical infrastructure, networks, systems etc. with examples. 
\item 
Third para
-	How cyberattack are being crafted? Here talk about use of GAIMS etc to launch sophisticated attack with examples. Talk about attackers’ strategies (evasion, deception etc) as well. 
\item 
Fourth para
-	Discuss how such attack can be prevented or analyzed in case of successful attack. Discuss our motivation of using CKC as a baseline to get better visibility into attack surface and attack vectors. Educate readers our focus is to only look at generative capabilities in CKC and why this is important. 
\item 
Fifth paragraph:
-	Talk about how we can defend against defense-aware adversary. Talk about we propose such and such defensive strategy. Etc .
\item 
Write Major Contribution
\begin{itemize}
\item A
\item B
\item C
\item D etc. 
\end{itemize}
\item 
Lastly, state what we will be explaining in  next sections. 
\end{itemize}
\end{comment} 

%\subash{1st para should be a story about cyber attacks ... wht are cyber attacks with examples...need to build up a story as to why we need to know more about offensive Gen AI... give example of CPS, Critical Infrastructure...and attack on them...}

\begin{comment}
\IEEEPARstart{G}{}enerative AI models (GAIMs)  are rapidly transforming the way we communicate, create, and work. 
All aspects of society will be affected by their consequences, from business development to medicine, from education to research, and from programming to entertainment.
There is great potential in GAIMs, however, they are also accompanied by significant risks. 
Presently, millions of people rely on them to create human-level text (e.g., ChatGPT, soon Bard, and Luminous), images (e.g., DALL-E 2, Steady Diffusion), videos (e.g., Synthesia), or audio (e.g., MusicLM), with more options on the way \cite{glaese2022improving, shuster2022blenderbot, scao2022bloom}.
It is likely that they will soon be incorporated into employment tools that rank and reply to job candidates, or into hospital administration applications that draft patients based on case histories.
As such, multi-model decision engines free up time for professionals to concentrate on important matters, such as actual patient treatment, and thereby might help allocate resources more effectively and more fairly.

Errors, on the other hand, will be expensive and risks varying from discrimination and privacy to offensive material must be handled properly \cite{zuiderveen2020strengthening, lee2021application, aung2021promise}.
GAIMs are exploding all over the place, essentially altering everything we know about how cybercriminals create and execute attacks with greater speed and variety.
By combing generative AI and diffusion models, AI-powered technologies can modify the appearance of video and voice.
Currently, GAIMs are already capable of delivering fake news %\ivan{Disinformation is false information which is deliberately intended to mislead}, 
manipulating user behavior, and creating harmful speech at an unprecedented level \cite{marcus2023skeptical, beuth2023chatgpt, bergman2022guiding, mirsky2022threat}.
Moreover, attackers could use them to mislead autonomous driving vehicles \cite{kurakin2018adversarial, eykholt2018robust, xie2017adversarial}  or hijack voice-controlled intelligent agents \cite{carlini2016hidden, zhang2017dolphinattack, cisse2017houdini}.
They will almost certainly be employed for cyberattacks, with disastrous repercussions for organizations.
As a consequence, the discussion over how to control (or not to regulate) generative models is heating up \cite{edwards2022regulating, hacker2023understanding, gutierrez2022proposal, goldstein2023generative}.
       
\hl{The development of defensive generative models is accompanied by the evolution of intrusion strategies.} \subash{is this statement true??? citation???} \milan{I'll add citation}
An especially concerning trend in malware evolution is the emergence of self-adaptive malware capable of changing its behavior to avoid detection by a security mechanism.
\cite{wu2019evading} proposes a deep Q-learning method to bypass botnet detection models by controlling the network traffic flow generated by the botnets.
The use of Generative Adversarial Networks (GAN) by Shi et al. \cite{shi2018generative} to synthesize training data for exploratory attacks and causative attacks on a real online classifier for text subjectivity analysis.
Using deep neural networks and GANs to accelerate the prediction model training, Erpek et al. \cite{erpek2018deep} propose an effective method for jamming attacks on wireless communication channels.
Rigaki and Garcia use GANs to mimic Facebook chat traffic profiles in the Command and Control (C2) channel of a Remote Access Trojan malware \cite{rigaki2018bringing}.
A GAN-based attack method is also proposed by Lin et al. \cite{lin2022idsgan} in which the generator computes the adversarial network traffic features used to attack a Black-box security mechanism.
Among the different methods proposed in \cite{wu2019evading, rigaki2018bringing, lin2022idsgan}, the \textit{adversarial attack} can be categorized into a special class of attack targeting the security detection model built using machine-learning (ML).  

As the name implies, an adversarial attack is an action that (intentionally) causes classification error in an ML algorithm by perturbing its input feature point.
The perturbed feature is referred to as the adversarial feature, or the adversarial case is similar to the initial feature in terms of distance metric (e.g., Euclidean distance).
The adversarial feature of a malicious network traffic flow can be computed using an adversarial attack algorithm.
Once the value of an adversarial feature has been determined, the malware can alter how it generates network traffic flow to match the calculated value, causing the security detection system to classify the modified traffic flow as benign traffic. 
The malware has a high chance of retaining its invasive functionality due to the small magnitude of the feature value perturbation.
However, the specific features and behavior of the adversarial attack have yet to be thoroughly investigated and documented.
Though some phases of an adversarial attack (e.g., delivery) are similar to other malware samples, some other phases (such as its installation, propagation, and persistence) are different.
We believe that the lack of a systematized and comprehensive reference detailing speciﬁc features of generative AI attacks is among the important barriers to the introduction of effective preventive and detective methods.
This is due to the fact that security analysts would be able to detect these attacks in their early stages only if they are aware of the speciﬁc features (e.g., weaponization, exploitation, or installation methods) of generative AI attacks. 
A comprehensive taxonomy would help in identifying different generative models, classifying them based on their known features, and providing a dedicated course of action for each category.

%A number of scholars have developed taxonomies to classify cyber-attacks using different models [7-11]. 
%For example, Chapman et al. [7] introduced a taxonomy based on the different types of attacks used by cyber-attackers and described the access requirements for a successful attack. 
%Note, however, that their model does not consider the different stages of an attack, and it cannot guide cyber-defenders in dealing with sophisticated campaigns. 
%The taxonomy proposed by Hansman and Hunt [8] is multi-dimensional, having categorizations for attack vectors, targets, vulnerabilities, and payloads. 
%Nonetheless, the taxonomy only describes specific campaigns run by different advanced attackers such as the Code Red Computer worm, not the overarching activities of different actors.

%Advance hackers conduct thorough studies on their targets before launching a well-planned attack in order to maximize the effect, such as identifying data/assets of interest with the goal of getting the most valuable information while reducing the risk of disclosure.
%The salient features of attackers are: (1) well-researched, pre-determined with a clear goal \cite{decker2013communications}; (2) use/modify sophisticated tools and techniques to exploit vulnerabilities, particularly zero-day vulnerabilities, in systems and computing devices \cite{chen2014study}; (3) developing a strategy for monitoring and exfiltrating data from a specific target via both cyber and physical means \cite{chen2014study}; and (4) sophisticated, well-organized, well-resourced campaigns \cite{chen2014study}.

This motivated us to provide, to the best of our knowledge, the taxonomy of generative models. 
To this end, we provide the reader with detailed information about the generative model's lifecycle; enabling researchers to ﬁgure out how a criminal launches a generative model attack and infects a victim, how self-generative malware hides itself, as well as the actions that malware performs on the victim’s machine. In order to provide such information in a more understandable and systematized manner, we have adapted the Cyber Kill Chain (CKC) \cite{hutchins2011intelligence} model to our generative model taxonomy to describe phases of computer network intrusions and delineating the steps of a cyber attack. %\ivan{the last sentence needs to be cleaned up... "and later on adapted for..."}
Our motivation behind aligning our proposed taxonomy with the CKC model is to provide information in detail about each step that the attacker must accomplish in order to achieve the goal, as the attack would fail otherwise.
For each step, our defensive strategies would improve the Cyber Security Operation Center (CSoC) analyst(s)  grasp of the proof they need to look for in order to detect the attack and safeguard network systems.

The major contributions of our research are:
\begin{itemize}
    \item We propose a systematized analysis and taxonomy of generative models inspired by XXX \milan{need to complete by Subash}  
    \item We identify attack strategies employed by the adversaries to launch a more sophisticated and stealthy, attack by examining Cyber Kill Chain (CKC) framework \cite{hutchins2011intelligence}.
    \item We propose proactive defense strategies for the defenders to implement appropriate strategies that can detect and respond to these evolving threats.
\end{itemize}
Our proposed defensive taxonomy could be used by many organizations which are using CKC in their day-to-day cyber defense planning to address the risk of generative model attacks by finding out what are the types of attacks and features of the generative attack that they should look for in their analysis.

%In this paper, in order to help researchers and security analysts in understanding the generative attack and finding efficient detection mechanisms, we provide a systematized analysis and taxonomy of generative models and their defense strategies. 
%As a systematization methodology, we consider Cyber Kill Chain (CKC) framework \cite{hutchins2011intelligence} and align the behavior of the proposed taxonomy with the offensive steps of a cyber intrusion as described in the CKC framework (which we explain in Section \ref{kill_chain_risk}). 
%Our proposed taxonomy could be used by many organizations which are using CKC in their day-by-day cyber defense planning to address the risk of generative model attacks by finding out what are the types of attacks and features of the generative attack that they should look for in their analysis. 
%After obtaining such information about the structure of the intrusion, the reader needs to know how to defend against each phase of the intrusion attempt. 
%In line with the Lockheed Martin Course of Action (CoA) matrix [20], we provide the required information for the defenders to implement appropriate strategies (see Section \ref{strategy}). 

The remainder of the paper is organized as follows: In Section \ref{generative} we provide the required background knowledge on Generative AI and how synthetic data can be generated from certain inputs. We also present our Generative Model taxonomy. 
Section \ref{strategy} discusses the attack strategies that can effectively help cyber-attacks effectively to help CSoC analysts curb cyber threats. 
In Section \ref{kill_chain_risk} we provide the required background knowledge on the CKC framework, which traces the various stages of a cyber-attack, identifies vulnerabilities, and assists security teams in preventing attacks at each level of the chain. 
Section \ref{defstrategy} discusses defense strategies against attack strategies of cyber attacks, as well as showcasing the course of action for some well-known generative attacks effectively.
Finally, Section \ref{conclusion} presents our conclusion and outlines possible future work.

\end{comment}


% Survey Generative ai
% https://arxiv.org/pdf/2301.04655.pdf
% application and models og Generative AI - https://www.sequoiacap.com/article/generative-ai-a-creative-new-world/
% paper - https://dl.acm.org/doi/pdf/10.1145/3491101.3503719 --- GenAICHI: Generative AI and HCI
%https://tinyurl.com/82u3h2ek ---- A comprehensive survey and analysis of generative models in machine learning
%- Google  Phenaki -----
% https://arxiv.org/abs/2210.02399 

%The term "generative AI" is used to describe the use of unsupervised and semi-supervised machine learning algorithms to generate synthetic data from existing data such as text \cite{}, audio \cite{} and video files \cite{}, images\cite{}, and code \cite{}.


%Most of the generative models are based on the principle of maximum likelihood. The idea is to choose the parameters for the model that maximize the likelihood of the training data. Furthermore, generative model tries to address the density estimation problem, a core problem in unsupervised learning. 


%As indicated in Fig \ref{fig: Generative_models} of the taxonomy of generative models, there are two types of density estimation: explicit density estimation and implicit density estimation.



%To address this issue two approach has been suggested in the body of literature; first is to design model to have a tractable density function, second is to design a learning algorithm based on a computationally tractable approximation of an intractable density function \cite{goodfellow2020generative}.

%Deep Generative models are based on density estimation function: explicit and implicit as illustrated in Fig \ref{fig: Generative_models} \todo{THe figure needs to be integrated in the text. What is the figure about? write that in text.}. Example \todo{these are not examples/models, more like techniques} of generative models with explicit density estimation are Fully Visible Belief Nets (FVBN) \cite{frey1995does} and Nonlinear Independent Component Analysis (NICA). These models provides explicit parametric specification of the distribution of an observed random variable $x$ by defining a log-likelihood function $log q _\theta (x)$ with parameters $\theta$. Utilizing simple functional forms of probability distribution and typically applied to limited numbers of variables, these models have historically proved effective for traditional statistics. However, with the emergence of Deep Learning (DL), the focus of study has shifted to learning models with relatively complex functional forms, because when DL is used for synthesis, the corresponding density function may be computationally intractable \cite{goodfellow2020generative}. %To address this issue two approach has been suggested in the body of literature; first is to design model to have a tractable density function, second is to design a learning algorithm based on a computationally tractable approximation of an intractable density function \cite{goodfellow2020generative}. Nevertheless, these approaches have proven to be difficult and, in some cases, generating samples using these method is very expensive. For example, FVBN uses chain rule to decompose a probability distribution and the samples are generated sequentially: $x{_1},x{_2}, …x{_n}$ with computational cost of $O(n)$. 


\begin{comment}
\begin{equation}
p_{\text {model }}(\boldsymbol{x})=\prod_{i=1}^n p_{\text {model }}\left(x_i \mid x_1, \ldots, x_{i-1}\right)
\end{equation}

\begin{equation}
p_x(\boldsymbol{x})=p_z\left(g^{-1}(\boldsymbol{x})\right)\left|\operatorname{det}\left(\frac{\partial g^{-1}(\boldsymbol{x})}{\partial \boldsymbol{x}}\right)\right|
\end{equation}

%Variational approximations is give by: 
\begin{equation}
\mathcal{L}(\boldsymbol{x} ; \boldsymbol{\theta}) \leq \log p_{\text {model }}(\boldsymbol{x} ; \boldsymbol{\theta})
\end{equation}
\end{comment}


%\todo{the heading is language models but your exampleas are generic and not just limited to language}
%GMs is currently applied in several domains, for example BERT \cite{devlin2018bert}, GPT-3 \cite{brown2020language} are state-of-the-art transformer-based text generator models. 

%Other use of GMs include text-to-image: DALL-E 2 \cite{ramesh2021zero}, Imagen \cite{kingma2021variational}, \ivan{Maybe add Midjourney} text-to-video: Phenaki \cite{villegas2022phenaki}, text-to-3D: DreamFusion \cite{poole2022dreamfusion}, text-to-code: Codex \cite{chen2021evaluating}, text-to-audio: AudioML \cite{borsos2022audiolm}, Wishper \cite{radford2022robust}, image-to-text: VisualGPT \cite{chen2022visualgpt}. \todo{this colon list wont do, needs to be converted to a papragraph}



%\ivan{might need to change to "Starting with the next section..." since the whole paper deals with offensive strategies using generative AI.}In the section that follows, we describe how generative models can be used as offensive artificial intelligence by examining the cybersecurity kill chain \cite{hutchins2011intelligence}, a framework for understanding the structure of a cyberattack in terms of five stages: research and reconnaissance, access and penetration, delivery, exploitation, C2 action, and objectives.

\begin{comment}
    
The na
\subsubsection{Text to Text }
ChatGPT3 (transformer based model, training however is made through Reinforcement Learning), Lambda (This model is for dialog application, trained on dialogues, again it is also transformer based model.) ,Peer


\subsubsection{Text to Image }
   DALL-E 2 (working CLIP and Diffusion models), Imagen (Transformers and Diffusion), Stable Diffusion (Latent Diffusion Models), Muse
DALL·E 2, created by OpenAI, is able to generate original, genuine
and realistic images and art from a prompt consisting on a text description .

\subsubsection{Text to Video }
Phenaki (Video synthesis, components of the model -> C-ViViT encoder, transformer and video generator),  Soundify (uses CLIP (nn with 0-shot image classification capabilities), this model has 3 parts such as classification, synchronization, and mix)


\subsubsection{Text to 3D }
DreamFusion, Magic3D (Slower than Dreamfusion, long processing times, Low quality, developed by NVIDIA, Again diffusion models), MDM


\subsubsection{Text to Code }
Codex (Finetuned using GPT-3,), Alphacode


\subsubsection{Text to Audio }
Audio ML, Jukebox (uses VQ-VAE architecture ), Wishper

\subsubsection{Image to Text }
Flamingo, VisualGPT

\end{comment}


\begin{comment}
Most of the Generative model address density estimation problem, a core problem in unsupervised learning as depicted in Fig \ref{fig: Generative_models}. There exist two types of density estimation such as explicit density estimation  and implicit density estimation. The first one explicitly defines and solve for $\tilde p_{model}(x)$ whereas the later one learns model that can produce a sample from $\tilde p_{model}(x)$ without explicitly defining it.

Generative AI can be defined as an AI system that uses exist-
ing media to create new, plausible media [37, 38 , 46 , 47, 56 ]. This
scope is broad, and the generative potential of AI systems varies
greatly. Over the last decade, we have seen a shift in methodol-
ogy moving from expert systems based on patterns and heavy
human curating [e.g., 16 , 22 , 40] towards stochastic and generative
models such as Generative Adversarial Networks (GANs) that use
big data to produce convincingly human-like results in various
domains [14, 19, 47, 59].

Generative AI refers to a type of AI that is able to generate new content, such as text, images, or music, based on certain inputs. This is often accomplished using a type of machine learning model called a generative model, which is trained on a large dataset of examples and can then generate new examples that are similar to the ones it was trained on. For example, a generative model might be trained on a dataset of images of faces and then be able to generate new, previously unseen faces that look realistic.

\end{comment}

%NVIDIA’s BioNeMo is a framework for training, building and deploying large language models at supercomputing scale for generative chemistry, proteomics, and DNA/RNA. --- Website === https://hbr.org/2022/11/how-generative-ai-is-changing-creative-work



%Furthermore, by automating the obfuscation process, they can automatically generate obfuscated versions of their malware that exhibit higher levels of sophistication and resistance to reverse engineering. This makes it more difficult for security analysts to comprehend the malware's behavior, extract Indicators Of Compromise (IOCs), or develop effective detection systems. 


%\subash{ => Milan ::: I think we need to explain how attacker can use game theoritc approach to adapt and penetrate against new security measures. One example can be generating synthetic adversarial samples that are hard to differenciate. Give example of generator and discriminator ... e.g player a is defese system player b is attacker. Player uses GANs to craft realistic sample that is hard to differentiate (usually by feed back they get from disrciminator and updating generator (back propagation may be)  to make realistic sample.) The content should be reworded with this theme in mind...I guess. for e.g. How to adapt against Proactive defense systems?? Other areas could be ...how to adapt when in black box attack settings? Another could be how to attak against white box settings?? This three areas might be better in this strategy. Maybe this paper https://tinyurl.com/2mf5r3ua can be helpful here}
\begin{comment}
\subash{our intention here is to showcase how are attackers evolving in crafting sophisticated attacks...matter of fact how are they adapting day to day...game theoretic approach is good. I think you need to refer back to my previous comment ....also i think you need to use word "Adaption" more often in the text????}
\hl{Milan work here} Adaptive attacks have (rightfully) become the de facto norm for assessing defenses against adversarial instances.
The attacks involving adaptation can gain access to sensing and actuation computing platforms (i.e., approach and adapt) and manipulate system measurement data, and control input commands (i.e., penetrate security measures) to severely compromise system performance and integrity.
Adaptive attacks are composed of reusable building blocks that can be formalized in a search space and used to discover attacks for unknown defenses automatically. 
One example can be generating synthetic adversarial samples that are hard to differentiate.
On the other hand, adaptive control relies on the potential of parameter adjustments to assure the security and reliability of closed-loop systems in the presence of various unknown faults and attacks.
%There has been a significant uptake of evaluations against adaptive attacks, i.e., attacks that were specifically designed to target a given defense—the ratio of defenses evaluated against adaptive attacks has increased from close to zero in 2017 \cite{carlini2017adversarial} to one-third in 2018 \cite{athalye2018robustness} and to nearly all of them today.

The adversary can use a game theoretical approach to launch attack. 
For example, there are two players in the game, player A is the attacker and player B is the defender. 
The stealthy, persistent, and deceptive features result in incomplete information about the attacker's to the defender.
The attacker, i.e., the adversarial user, disguises himself as the legitimate user, thus the defender does not know about the user. 
The set of the user’s type can also be non-binary and incorporate different groups when their attack tools and targeted assets are different \cite{lemay2018survey}.
The attacker uses GANs to craft a realistic sample that is hard to differentiate (usually by the feedback they get from a defender and updating generator (back propagation) to make a realistic sample.
At the same time, the defender makes decisions based on the output of an imperfect detection system. 
Adversaries may employ generative models to launch Thwart DoD attacks \cite{khanna2011adaptive}, whereby pose an elevated threat to the reliability of the Internet.
Such attacks may occur at various levels of the protocol stack and harm both routers and hosts. 
Numerous attacks try to drain precious resources (e.g., CPU, memory, disk) by making bogus requests from one or more attacker-controlled sites \cite{moore2006inferring}. %\cite{TwitterF45:online}, \cite{Georgiaa66:online}. 
The time necessary to process these requests either degrades the service to available consumers to an unacceptable degree or causes expensive overprovisioning by the service provider. 
Examples of potentially susceptible services include IKE key exchanges for gateway security association establishment \cite{kaufman2005internet}, traditional and digitally signed DNS services \cite{eastlake1999domain}, massive file retrievals from Web servers, and computationally costly query processing at database front ends.
\end{comment}



==> resources.tex <==
% Please dump and resource here if you think it might be useful for us. -Thank you.


%----------################_--------------------------
% The AI-Based Cyber Threat Landscape: A Survey
%https://dl.acm.org/doi/pdf/10.1145/3372823 

%----------################_--------------------------


%resource for good writeup : https://dl.acm.org/doi/pdf/10.1145/3422622
